Sensor Setups for State and Wind Estimation for Airborne Wind Energy Converters

An unscented Kalman filter with joint state and parameter estimation is proposed for aerodynamics, states and wind conditions for airborne wind energy converters. The proposed estimator relies on different measurement setups. Due to the strict economic constraints of wind energy converters, the sensor setups are chosen with minimal cost and reliability issues in mind. Simulation data with a high fidelity system model and experimental tests using flight data, together with wind measurements obtained using a lidar system for altitude wind measurements, are used for validation. The data was obtained during test flights of the EnerK\'ite EK30, an airborne wind energy converter currently in research operation in Brandenburg, Germany. Feasible accuracies were achieved even with the simplest of setups and illustrate the gain achievable by airborne sensors. Additionally, the results encourage further research into use of the obtained wind estimates for site assessment.

==> measModel.tex <==
\section{Measurement Model}
